Commit: Online Groups with Participation Commitments

In spite of efforts to increase participation, many online groups struggle to survive past the initial days, as members leave and activity atrophies. We argue that a main assumption of online group design -- that groups ask nothing of their members beyond lurking -- may be preventing many of these groups from sustaining a critical mass of participation. In this paper, we explore an alternative commitment design for online groups, which requires that all members commit at regular intervals to participating, as a condition of remaining in the group. We instantiate this approach in a mobile group chat platform called Commit, and perform a field study comparing commitment against a control condition of social psychological nudges with N=57 participants over three weeks. Commitment doubled the number of contributions versus the control condition, and resulted in 87% (vs. 19%) of participants remaining active by the third week. Participants reported that commitment provided safe cover for them to post even when they were nervous. Through this work, we argue that more effortful, not less effortful, membership may support many online groups.

==> figures/fulfill_chat.tex <==
\begin{figure}[htb]
  \centering
  \begin{subfigure}{0.2\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/no_fulfilled.png}
  \end{subfigure}
  % \hspace{0.5 cm}
  \begin{subfigure}{0.2\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/before_send_chat.png}
  \end{subfigure}
  \hspace{1 cm}
  \begin{subfigure}{0.2\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/one_fulfilled.png}
  \end{subfigure}
  % \hspace{0.5 cm}
  \begin{subfigure}{0.2\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/after_send_chat.png}
  \end{subfigure}
    \hspace{1 cm}
  \begin{subfigure}{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/two_fulfilled.png}
  \end{subfigure}
  % \hspace{0.5 cm}
  \begin{subfigure}{0.24\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/more_sent_chat.png}
  \end{subfigure}
  
  \caption{Paired fulfillment information and chat behavior.}
  \label{fig: fulfill correspond}
\end{figure}


==> tables/quant_comparison.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}

\begin{table}[htb]
\begin{center}
\begin{tabular}{l l l}
\hline
Measure & Commit & Slack Control \\
\hline\hline
Gini coefficient & 0.46 & 0.76\\
Total posts & 195 & 83\\
Total users & 8 & 15 \\
Median posts per user & 12.5 & 2\\
Minimum posts from user & 3 & 0 \\
\hline


\end{tabular}
\end{center}
\medskip
\caption{Comparison of participation in Commit and Slack control.}
\label{table: quant comparison}
\end{table}

==> tables/question_themes.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}

\begin{table}[htb]
\begin{center}
\begin{tabular}{l p{8cm}}
\hline
Theme & Example Question(s) \\
\hline\hline
Perceived activity level & What is your estimation of your own activity level? Others in the group? \\
Value of contribution & Did they consider the impact of their posting on others? \\
Comfort-level & Was it ever awkward to post? Were they ever left hanging? \\
Pressure and obligation & Did they feel obligated to post? Why? \\
Perception of others & Did they think about how others perceived their content? \\
Group culture & What did the group feel like? \\
Critical incident & Was there a memorable moment? \\
Commitment mechanism & What did they feel when they committed \\
\hline


\end{tabular}
\end{center}
\medskip
\caption{Semi-structured interview themes and example questions.}
\label{table: interview questions and themes}
\end{table}
